On the Succinctness of Alternating Parity Good-for-Games Automata

We study alternating parity good-for-games (GFG) automata, i.e., alternating parity automata where both conjunctive and disjunctive choices can be resolved in an online manner, without knowledge of the suffix of the input word still to be read. We show that they can be exponentially more succinct than both their nondeterministic and universal counterparts. Furthermore, we present a single exponential determinisation procedure and an Exptime upper bound to the problem of recognising whether an alternating automaton is GFG. We also study the complexity of deciding "half-GFGness", a property specific to alternating automata that only requires nondeterministic choices to be resolved in an online manner. We show that this problem is PSpace-hard already for alternating automata on finite words.

==> 6_cobuchi.tex <==
\newcommand{\sigmamove}{\sigma_{\mathit{move}}}
\section{Deciding GFGness of NCW via Two-Token Games}
\label{sec:G2-coBuchi}



The following theorem constitutes a step towards proving \cref{con:G2-to-GFG}. It also provides a simplified  \ptime algorithm for deciding whether an NCW is GFG: it suffices to solve $\Gt$.

\begin{theorem}
\label{thm:G2cobuchi}
A~nondeterministic~coB\"uchi~automaton~$\A$~is~GFG~if~and~only~if~Eve wins~$G_2(\A)$.
\end{theorem}

We give only a proof sketch conveying the main ideas of the construction, leaving the detailed proof to \cref{ap:G2-coBuchi}.
The proof is partly inspired by the construction from~\cite{BK18} for B\"uchi automata, while techniques tailored to coB\"uchi automata from~\cite{KS15} are also used, and new insights allow to combine them.

Unfortunately, this result does not immediately extend to alternating coB\"uchi automata, because (contrary to the case of B\"uchi automata), the box automaton constructed for a coB\"uchi automaton may not be coB\"uchi any more.

It is straightforward that if an NCW $\A$ is GFG then Eve wins $G_2(\A)$ \cite{BK18}.  We thus assume that Eve wins $G_2(\A)$ and show that $\A$ is GFG.
\Subject{Global proof scheme}
Let us start by recalling the main proof scheme of \cite{BK18}, showing that for all NBW $\A$, if Eve wins $G_2(\A)$ then $\A$ is GFG:
\begin{itemize}
\item For every $k\in\Nat\setminus\{0,1\}$, Eve wins $G_2(\A)$ if and only if Eve wins $G_k(\A)$, a game where she has one token and Adam has $k$ tokens.
%\item Eve winning $G_2$ guarantees that the automaton can be put into a normal form, called \emph{residual automaton} that guarantees certain properties of all partial runs.
\item We assume, towards contradiction, that the automaton is not GFG, and we fix a finite\=/memory strategy $\stratA$ for Adam in the letter game of $\A$. This strategy chooses letters such that the produced word $w$ is always in $L(\A)$. Moreover, the finite memory of $\stratA$ guarantees additional structure on the run-DAG of $\A$ on $w$.
\item We describe a strategy $\sigmamove$ to move a fixed number $N$ of tokens in $\A$, such that any word produced by $\stratA$ will be accepted by one of the $N$ tokens.
\item Finally, we build a strategy $\stratE$ for Eve in the letter game of $\A$, moving $N$ virtual tokens in her memory according to $\sigmamove$, and playing her winning strategy $\sigma_N$ in $G_N(\A)$ against them. The play yielded by $\stratE$ playing against $\stratA$ will be winning for Eve, contradicting the fact that $\stratA$ is a winning strategy in the letter game.
\end{itemize}


\begin{remark}
The above proof from \cite{BK18} can also handle directly the \emph{generalised B\"uchi} condition, which is a union of B\"uchi conditions. The adaptation is straightforward. So the $G_2$ conjecture also holds for generalised B\"uchi automata.
\end{remark}


\Subject{Switching to the coB\"uchi condition}
The goal is to use the same proof scheme. However the strategy $\sigmamove$ will be more involved. Indeed, for the B\"uchi condition, it was enough to take $\sigmamove$ to be a strategy spreading tokens evenly at each nondeterministic choice. This is no longer true for the coB\"uchi condition, and the main challenge here consists in building a strategy $\sigmamove$ with the same properties.
The following ideas are inspired by \cite{KS15}:
\begin{itemize}
\item We show that the automaton $\A$ can be taken in a form that guarantees properties related to the winning region of $G_2(\A)$ and the structure of the graph of accepting transitions.
\item Thanks to this, we show that there is a subset $S$ of states of $\A$ and a deterministic transition function $\deltadet$ such that any word $w\in L(\A)$ is ultimately accepted from a state of $S$ via the run yielded by $\deltadet$, without any rejecting transition.
\end{itemize}

We also provide a new construction: we use the fact that Eve wins $G_k(\A)$ for every $k\in\Nat$ to build a ``limit strategy'' $\sigmainf$ in the letter game of $\A$. This strategy might build a rejecting run, but guarantees that for each state $p$ it reaches, and any number $k$ of tokens at reachable states $q_1,\dots,q_k$, the position $(p;q_1,\dots ,q_k)$ is in the winning region of $G_k(\A)$.\\

We are now ready to build the strategy $\sigmamove$, which is the only missing piece to complete the proof.
We take a big number $N$ of tokens that depends on the size of $\A$ and on the size of the memory of Adam's strategy $\stratA$.
The strategy $\sigmamove$ moves these $N$ main tokens according to $\sigmainf$ until, one by one, they become \emph{active} and deviate from $\sigmainf$ to attempt to build an accepting run. To do so, the current active token will play $\sigma_{|S|}$, the winning strategy in $G_{|S|}$, against $|S|$ virtual \emph{deterministic tokens}. These $|S|$ tokens start from the states of $S$ that Adam could have reached, and move deterministically according to $\deltadet$. We use here the fact that $\sigmainf$ was built so that the active token is in a position to win $G_{|S|}(\A)$. If a deterministic token encounters a rejecting transition, it is considered \emph{dead}. If all deterministic tokens are dead, we reached a \emph{breakpoint}: a new main token becomes active, and deviates from $\sigmainf$ by starting to play $\sigma_{|S|}$ against $|S|$ new virtual deterministic tokens. On the other hand, if at least one of these deterministic tokens stays alive forever, then our currently active token will build an accepting run by correctness of $\sigma_{|S|}$. We show that this must happen eventually, as otherwise there are $N$ ``breakpoints'', contradicting the fact that the finite-memory strategy $\stratA$ only builds words in $L(\A)$. This means that the global strategy $\sigmamove$ is correct: one of the $N$ main tokens will always build an accepting run, providing the input word has been produced by $\stratA$.
The behaviour of tokens is illustrated in \cref{fig:tokens}.

\begin{figure}[H]
\centering
\includegraphics[scale=.5]{runs.pdf}
\caption{An illustration of the behaviour of tokens in the memory structure of the strategy $\stratE$. Awaiting main tokens are represented in black, active main tokens in green, and alive deterministic tokens in red. Breakpoints are represented by dashed vertical lines.}
\label{fig:tokens}
\end{figure}

Finally, to win the letter game against $\tau$, Eve moves her token by simulating her strategy in $G_N(\A)$ against $N$ virtual tokens moving according to $\sigmamove$. Then, as $\tau$ plays a word in $L(\A)$, one of the $N$ virtual tokens is guaranteed to follow an accepting run, so Eve's token will also follow an accepting run. This contradicts the assumption that $\tau$ is a winning strategy for Adam, and proves that $G_2$ indeed characterises GFGness of NCW.


==> AP_6_cobuchi.tex <==

\section{Appendix of \cref{sec:G2-coBuchi}}
\label{ap:G2-coBuchi}

In this section we show that a nondeterministic coB\"uchi automaton $\A$ is GFG if and only if Eve wins $G_2(\A)$. This constitutes a step towards \cref{con:G2-to-GFG}.

Let us fix an NCW $\A=(\Sigma,Q,\iota,\delta,\alpha)$ with a transition function $\delta\colon Q\times\Sigma\to 2^Q$ and a set of accepting transitions $\alpha\subseteq Q\times\Sigma\times Q$ .

We use the following standard extensions of the transition function $\delta$:
\begin{itemize}
\item $\overline{\delta}:2^Q\times\Sigma\to2^Q$ is defined by $\overline{\delta}(X,a)=\bigcup_{p\in X} \delta(p,a)$.
\item $\delta^*:\Sigma^*\to 2^Q$ is defined by induction: $\delta^*(\varepsilon)=\{\iota\}$, and $\delta^*(ua)=\overline{\delta}(\delta^*(u),a)$.
\end{itemize}

First, let us recall results on $G_2(\A)$ from \cite{BK18} that are valid for coB\"uchi automata.

\begin{lemma}[\cite{BK18}]\label{lem:GFGtoG2} 
If $\A$ is GFG then Eve wins $G_2(\A)$. 
\end{lemma}


\begin{lemma}[\cite{BK18}]\label{lem:ktokens}
If Eve wins $G_2(\A)$ then for all $k\in\mathbb N$, Eve wins $G_k(\A)$.
\end{lemma}

From now on, we assume that Eve wins $G_2(\A)$, and aim at proving that $\A$ is GFG.

\subsection{Normalisation}

Along the proof, we will change $\A$ to a different automaton $\A'$, while ensuring that if $\A'$ is GFG then so is $\A$. We will then show that $\A'$ is indeed GFG, reaching the required result.

We will use the following operations to change $\A$:
\begin{itemize}
\item \emph{$G_2$-restriction}: We ``clean'' $\A$ to only have states from which Eve wins the $G_2$ game, namely restrict it to the states $Q' =  \{q \St $ Eve wins $G_2(\A^q) \}$, and remove the remaining states and transitions involving them.

\item \emph{Reachability labelling}: 
States occupied by tokens at a given time in a token game on $\A$ are always ``co-reachable'', namely there is a word on which $\A$ can reach all of them. Therefore, augmenting the states of $\A$ with the set of currently reachable states may intuitively help in analysing token games on $\A$. We accordingly define the NCW $\A'=(\Sigma,Q',\iotar,\delta',\alpha')$ that behaves like $\A$, but with an additional component storing the set of states reachable on the prefix read so far. (Cf.\ the ``augmented subset construction'' of \cite{BK12}.)

That is, we define the components of $\A'$ as follows: $Q'=\{(p,X)\in Q\times 2^Q\mid p\in X\}$, $\delta':Q'\times\Sigma\to 2^{Q'}$ defined for every 	
state $(p,X)$ and letter $a\in\Sigma$ by $\delta'((p,X),a)=\{(p',X')\mid p'\in\delta(p,a), X'=\overline{\delta}(X,a)\}$, and the accepting transitions are 	
$\alpha'=\{\trans{(p,X)}{a}{(q,X')}\mid a\in\Sigma, \trans{p}{a}{q}\in\alpha, X'=\overline{\delta}(X,a)\}$.
Notice that the second component evolves deterministically, and that $L(\A')=L(\A)$.
	
\item \emph{Acceptance tuning}: For a coB\"uchi automaton $\A$, we want to normalise $\A$ to only have accepting transitions that can be used infinitely often in an accepting run. We therefore define the accepting transitions of $\A'$ to be the ones that are accepting in $\A$ and are part of a maximal strongly connected component of accepting transitions of $\A$. In other words, all transitions $\trans{p}{a}{q}$ for which there is no path of accepting transitions from $q$ to $p$ in $\A$ are made rejecting. We will call these latter transitions \emph{SCC-changing}.
\end{itemize}

We first show that the $G_2$-restriction allows Eve to win $G_2$ from every state. Notice that it is not trivial from the definition, as her $G_2$ winning strategy in $\A$ might upfront visit states that are then removed in the $G_2$-restriction.

\begin{lemma}
\label{lem:G2RestrictionPreserve}
Consider a nondeterministic coB\"uchi automaton $\A$ and the automaton $\A'$ that is derived from $\A$ by $G_2$-restriction. Then i) if Eve wins $G_2(\A)$ then she wins $G_2(\A'^{q'})$ for every state $q'$ of $\A'$, and ii) if $\A'$ is GFG then so is $\A$.
\end{lemma}

The proof of this lemma relies on the games $G_k(\A)$ as defined in \cref{rem:k-token-nondet}. We will additionally use the explicit shape of Eves strategies in these games, as in the definition of a strategy in memory from \cref{sec:Preliminaries}. For the sake of simplicity, we base that on the representation of the game $G_2(\A)$ (and analogously $G_k(\A)$) as in~\cite[Lemma~11]{BK18}. This means, that Eve's strategy in $G_k(\A)$ can be represented as $\stratE\colon M \times (\Sigma \times Q^{k+1})  \to Q$, where $M$ is the memory used by $\stratE$.

\begin{proof}\
\begin{enumerate}
\item[i)] Consider a state $p\in Q'$. By the definition of $Q'$, Eve wins $G_2(\A)$ from $(p;p,p)$, and by \cref{lem:ktokens} she also wins $G_4(\A)$ from $(p;p,p,p,p)$. Let $\stratE_4$ be her winning strategy that uses some memory structure $M_4$ as above.

We define a strategy $\stratE_2\colon M_4 \times (\Sigma \times Q^3)  \to Q$ of Eve in $G_2(\A)$, in which she plays like $\stratE_4$, assuming that the first two tokens of Adam in the 4-token game follow her token. The memory structure $M_4$ is maintained accordingly.
That is, when Eve's memory is $m$, her token is in state $p$, Adam's tokens are in states $q_1$ and $q_2$, and he chooses the letter $\letter$, we have $\stratE_2(m, \letter, p;  q_1, q_2)=\stratE_4(m,\letter, p; p, p, q_1, q_2)$. Observe that $\stratE_2$ is a winning strategy, since $\stratE_4$ is.

Now, it must be that all states visited by Eve's token in a play consistent with $\stratE_2$ are in $Q'$, as otherwise a play consistent with $\stratE_4$ can reach a position $(p; p, p, q_1, q_2)$, where  $q\in Q\setminus Q'$, from which Adam can win against $\stratE_4$, by diverting to a winning strategy of him in $G_2(\A)$ from $(q;q,q)$ with his first two tokens.

So $\stratE_2$ is actually a winning strategy in $G_2(\A')$ from $(p;p,p)$, as it never goes outside of $Q'$ (and this strategy even works when Adam is allowed to visit $Q$ and not only $Q'$).
			
			
\item[ii)]  It is enough to show that $L(\A)=L(\A')$, as then a winning strategy $\stratE\colon\Sigma^*\to Q'$ of Eve in the letter game for $\A'$ is also a winning strategy for her in the letter game for $\A$. (Every word generated by Adam is either not in their language, or followed by an accepting run of Eve in $\A'$, which is also an accepting run for her in $\A$.)
			
Assume toward contradiction that exists a word $w\in L(\A')\setminus L(\A)$.
We give a winning strategy for Adam in $G_3(\A)$, thereby contradicting \cref{lem:ktokens}.
Adam will play the word $w$, and make his first two tokens follow Eve's token, while the third token will follow an accepting run for $w$.
If Eve stays in $Q'$, then by the choice of $w$ she cannot build an accepting run, and Adam will win the play.
So Eve is forced to leave $Q'$ at some point, and the game reaches a position $(p;p,p,q)$ with $p\notin Q'$. By the definition of $Q'$, this means that Adam has a winning strategy $\stratA$ in $G_2(\A)$ from $(p;p,p)$. Adam can therefore stop playing $w$, and win by playing $\stratA$ against Eve with his first two tokens, while doing arbitrary choices with the third token. 
\end{enumerate}
\end{proof}

We continue with showing that reachability labelling and acceptance tuning do not change the $G_2$ winner, and if they produce a GFG automaton then so was the original one.

\begin{lemma}
\label{lem:OperationsPreserve}
Consider a nondeterministic automaton $\A$ and the automaton $\A'$ that is derived from $\A$ by acceptance tuning or reachability labelling. Then i) if Eve wins $G_2(\A^q)$ for every state $q$ of $\A$ then she wins $G_2(\A'^{q'})$ for every state $q'$ of $\A'$, and ii) if $\A'$ is GFG then so is $\A$.
\end{lemma}

\begin{proof}\
\begin{description}	
\item[Acceptance tuning]
Every run $r$ of $\A$ is also a run of $\A'$, and vice versa, and $r$ is accepting in $\A$ iff it is accepting in $\A'$. This is because any accepting run of $\A$ must eventually stay within a SCC of accepting transitions, and therefore avoid SCC-changing transitions. Therefore, the two required properties directly follow.

\item[Reachability labelling]\
\begin{enumerate}
\item[i)] Eve can simply use her winning strategy in $G_2(\A)$ --- the extra component of $\A'$ does not play any role in the acceptance condition, and evolves deterministically.

%\todo{again say something about the shape of strategies - this is not what we get from the definition!}
	
\item[ii)] Consider a winning strategy $\stratE'\colon\Sigma^*\to Q\times 2^Q$ of Eve in the letter game for $\A'$. Then Eve can win the letter game for $\A$, by using the strategy $\stratE\colon\Sigma^*\to Q$ that is derived from $\stratE'$ by ignoring the second component of the image. (Since the second component, consisting of the reachable states, evolves deterministically, Eve can compute it in the memory of her strategy.)	
\end{enumerate}
\end{description}
\end{proof}

\paragraph*{The automaton $\Ar$}

We continue with considering the automaton $\Ar=(\Sigma,\Qr,\iotar,\delr,\alpr)$ that is derived from $\A$ by first performing $G_2$-restriction, then reachability labelling, and finally acceptance tuning. We aim to show that it is GFG, which will show by \cref{lem:G2RestrictionPreserve,lem:OperationsPreserve} that $\A$ is GFG.

Notice that since Eve wins $G_2(\A)$, we have in particular $\iotar\in \Qr$.
In the sequel, we will use $\reach{q}$ to denote a state of $\Ar$ of the form $(q,X)$ with $q\in Q$ and $X\subseteq Q$.
The second component of a state in $\Qr$ (the $X$ in $(q,X)$ ) is deterministically determined (it is the subset construction on the part of $\A$ that was not removed in the normalisation). For a finite word $u$, we shall use $\delrr(u)$ to denote the component $X$ of a state $(q,X)$ reached by $\Ar$ reading $u$.

\subsection{Safety Game and Deterministic Runs}

We analyse the different regions of the automaton $\Ar$ with respect to states being ``safe'' for Eve and states from which she can have some ``partially deterministic'' choices. 

The following constructions and arguments refine the corresponding ones from~\cite{KS15}.

\begin{definition}
Consider an NCW $\C$ with a set $P$ of states. We define the \emph{safety game} $\Gsafe(\C)$ on $\C$ as in~\cite{KS15}: The game is played on $P^2$, and a turn from a configuration $(p,q)$ is played as follows:
\begin{itemize}
\item Adam chooses a letter $\letter\in\Sigma$,
\item Eve chooses a transition $\trans{p}{\letter}{p'}$
\item Adam chooses a transition $\trans{q}\letter{q'}$
\end{itemize}
If the transition $\trans{q}\letter{q'}$ chosen by Adam is rejecting then Eve wins the game immediately.
If $\trans{p}{\letter}{p'}$ is rejecting and $\trans{q}\letter{q'}$ is accepting, Eve loses the game immediately. Otherwise, the game moves to the position $(p',q')$ and a new round starts. Eve wins any infinite play. 
\end{definition}

The above game can again be defined as $(R_{A,\Sigma}\times \C)\times \overline{\C}$ with an appropriate winning condition.

Notice that $\Gsafe(\Ar)$ is a safety game for Eve, and in particular if she wins the game, she can do it with a positional strategy.

We will denote by $\Wsafe\subseteq \Qr^2$ the winning region of Eve in $\Gsafe(\Ar)$.
We show next that for every state in $\Ar$, there is a corresponding safe state sharing the same reachability\=/component. The proof is analogous to the proof of~\cite[Lemma~53 in Appendix~E.5]{KS15}, except that we additionally need to keep track of the component $X$ in the states in $\Qr$.

\begin{lemma}
\label{lem:safewin}
For all $(q,X)\in \Qr$, there exists $p\in Q$ such that $((p,X),(q,X))\in \Wsafe$.
\end{lemma}

\begin{proof}
Assume toward contradiction that there is a state $\reach{q}=(q,X)\in\Qr$ such that for all $p\in Q$, $((p,X),(q,X))\notin \Wsafe$. Since Eve wins $\Gt(\A)$ from each state, she also wins $G_1(\A)$ from $(\reach{q};\reach{q})$. We shall build a winning strategy $\stratA$ for Adam in $G_1(\Ar)$ from $(\reach{q};\reach{q})$, to obtain contradiction.

By the assumption on $\reach{q}$, we have $(\reach{q},\reach{q})\notin\Wsafe$. The strategy $\stratA$ of Adam will start by playing in order to win $\Gsafe$ from $(\reach{q},\reach{q})$.
This means that $\stratA$ guarantees to build a partial play $\trans{(\reach{q},\reach{q})}{u_1}{((p_1,X_1),(q_1,X_1))}$, where a rejecting transition has been seen only on Eve's moves.

Since $\reach{q}$ and $(q_1,X_1)$ are in the same SCC (accepting transitions do not change SCC), 
Adam can now play a word $v_1$ allowing his token to go back to $\reach{q}$.
By the acceptance tuning of $\Ar$, Adam can ensure that the partial run along $v_1$ sees only accepting transitions.

The play therefore reaches a position $((p_1',X), (q,X))$. Notice that the second component $X$ is the same, as it evolves deterministically according to the input word read so far (here $u_1v_1$).
By the assumption, we again have $((p_1',X), (q,X))\notin \Wsafe$. Adam can therefore reiterate the previous strategy: first play in order to win $\Gsafe$ from there, forcing Eve to witness a rejecting transition; then go back to $\reach{q}$ with his token, without seeing any rejecting transition on the loop. This reaches a position $((p_2',X), (q,X))$. Repeating this strategy ad infinitum constitutes the winning strategy $\stratA$, as Eve will be forced to see infinitely many rejecting transitions, while Adam will not see any.
\end{proof}

Let us define $\Ssafe\subseteq Q_r$ by $\Ssafe=\{ (p,X) \St ((p,X),(p,X)) \in\Wsafe\}$. 

From Lemma \ref{lem:safewin}, we deduce the following:
\begin{lemma}\label{lem:safepos}
For all $(q,X)\in Q_r$, there exists $p\in Q$ such that $((p,X),(q,X))\in\Wsafe$ and $(p,X)\in \Ssafe$.
\end{lemma}
\begin{proof}
Let $(q,X)\in Q_r$. By Lemma \ref{lem:safewin}, there exists $p_1\in Q$ such that $((p_1,X),(q,X))\in \Wsafe$. Again, there exists $p_2\in Q$ such that $((p_2,X),(p_1,X))\in \Wsafe$.
Iterating this construction builds a sequence $p_1,p_2,p_3,\dots$. Since $Q$ is finite, there exists $i<j$ such that $p_i=p_j$.
As it is shown in \cite{KS15} that $\Wsafe$ is transitive, we obtain that $p_i\in \Ssafe$ and $((p_i,X),(q,X))\in \Wsafe$. Therefore, taking $p=p_i$ concludes the proof.
\end{proof}
Notice that due to \cref{lem:safepos}, we have in particular that the initial state of $\Ar$, namely $(\iota, \{\iota\})$, is in $\Ssafe$, since $\iota$ is the only state of $\A$ that belongs to a state of $\Ar$ in which the second component is $\{\iota\}$.

We continue with another refinement of a result from \cite{KS15}:
\begin{lemma}\label{lem:safedet}
There exists a partial deterministic transition function $\deltadet\colon\Ssafe\times\Sigma\to \Ssafe$, where $\deltadet\subseteq \delr$, such that for all $w\in L(\Ar)$, there is a decomposition $w=uv$ and a state $s\in Q$, such that $(s,\delrr(u))\in \Ssafe$ and $\deltadet$ accepts $v$ from $s$ without any rejecting transition.
\end{lemma}

\begin{proof}
The function $\deltadet$ is defined by $\deltadet(\reach{p},a)=\sigmasafe(\reach{p},\reach{p},a)$, where $\sigmasafe$ is a positional winning strategy of Eve in $\Gsafe(\Ar)$.

Let $w=a_1a_2\dots\in L(\Ar)$, and $\rho=(p_0,X_0)(p_1,X_1)(p_2,X_2)\dots$ be an accepting run of $\Ar$ on $w$.
Let $k\in\mathbb N$ such that the last rejecting transition in $\rho$ occurs before position $k$. Let $u=a_1a_2\dots a_k$ and $v=a_{k+1}a_{k+2}\dots$, so $w=uv$.
After reading $u$, the run $\rho$ reaches a state $(p_k,X_k)$ with $X_k=\delrr(u)$.
By Lemma \ref{lem:safepos}, there exists $s_k\in Q$ such that $(s_k,X_k)\in \Ssafe$ and $((s_k,X_k),(p_k,X_k))\in\Wsafe$.

We now build by induction a sequence $(s_i)_{i\geq k}$, describing the run of $\Ar$ yielded by $\deltadet$ on $v$ from $(s_k,X_k)$. We show that this run does not contain rejecting transitions, thereby proving the Lemma.
To do so, we show the following invariant $(P_i)$: the run yielded by $\deltadet$ on $a_{k+1}\dots a_i$ does not contain rejecting transitions, and the remaining suffix $a_{i+1}a_{i+2}\dots$ can be accepted in $\Ar$ without rejecting transition from $(s_i,X_i)$.
For the induction base, we need to show that $(P_k)$ is true. The first part is trivial, and the second part follows from the fact that $((s_k,X_k),(p_k,X_k))\in\Wsafe$. Indeed, if from this position in $\Gsafe(\Ar)$, Adam plays $v$ and follows the suffix of $\rho$ from position $k$, Eve must accept $v$ from $(s_k,X_k)$ without seeing any rejecting transition, witnessing the wanted property.

For the induction step, assume $(P_i)$ holds on $(s_i,X_i)$, and let $(s_{i+1},X_{i+1})=\deltadet((s_i,X_i),\allowbreak a_{i+1})$ (recall that the second component evolves deterministically, so $\deltadet$ only chooses the first component $s_{i+1}$). We first need to show that this transition is well-defined and not rejecting.
From $(P_i)$, we know that $a_{i+1}a_{i+2}\dots$ can be accepted without rejecting transitions from $(s_i,X_i)$.
This means that $\sigmasafe((s_i,X_i),(s_i,X_i),a_{i+1})$ must not be rejecting, as otherwise the strategy $\sigmasafe$ would not be winning, since Adam could play an accepting transition from $(s_i,X_i)$ and immediately win the play. By definition of $\deltadet$, we obtain that the transition $\trans{(s_i,X_i)}{a_{i+1}}{(s_{i+1},X_{i+1})}$ is well-defined and accepting.
It remains to show the second part of $(P_{i+1})$, i.e., $a_{i+2}a_{i+3}\dots$ can be accepted from $(s_{i+1},X_{i+1})$ without any rejecting transition in $\Ar$.
Again, consider the play of $\Gsafe$ starting from $((s_i,X_i),(s_i,X_i))$ with Adam playing $a_{i+1}$ and Eve playing $\sigmasafe((s_i,X_i),(s_i,X_i),a_{i+1}))$ to $(s_{i+1}, X_{i+1})$.
If the suffix  $a_{i+2}a_{i+3}\dots$ cannot be safely accepted from $(s_{i+1},X_{i+1})$, then Adam can just play the accepting safe run from $(s_i,X_i)$ on $a_{i+1}a_{i+2}\dots$ (which exists by $P_i$), and win the game $\Gsafe$ against $\sigmasafe$. This is a contradiction, so $(P_{i+1})$ must hold.

This achieves the proof that $\deltadet$ builds a run without rejecting transition from $(s_i,X_i)$ on $v$.
\end{proof}

\subsection{Adam's Strategy $\stratA$ in the Letter Game}

Let us assume toward contradiction that although Eve wins $G_2(\Ar)$, $\Ar$ is not GFG, so Adam has a finite-memory winning strategy $\stratA$ in the letter game on $\Ar$.
Let $M$ be the memory used in $\stratA$, i.e., $\stratA$ has type $\Qr\times M\to \Sigma$ (together with a memory update function), and $m_0$ be the initial memory state.

We will explicit a property of $\stratA$ linked with the strategy $\deltadet$ from Lemma~\ref{lem:safedet}. 
%Recall that $\Ssafe\subseteq Q_{r}$ is defined as $\{\reach{p}\mid (\reach{p},\reach{p})\in\Wsafe\}$, i.e., based on the winning region of Eve in the safe game.

\begin{definition}\label{def:det-breakpoint}
Consider a word $u=a_1a_2\dots a_{|u|}\in\Sigma^*$. We say that positions $i_1<i_2<\dots<i_n$ are \emph{det-breakpoints} of $u$ if for every $j\in [1,n{-}1]$ and $s\in Q$ for which $(s,\delrr(a_1\dots a_{i_j}))\in \Ssafe$, the run yielded by $\deltadet$ from $(s,\delrr(a_1\dots a_{i_j}))$ on $a_{i_{j}+1}\dots a_{i_{j+1}}$ is not defined or witnesses a rejecting transition.
\end{definition}


\begin{lemma}\label{lem:taubreak}
There is a constant $N$ depending only on $\Ar$ and $M$, such that if $u$ is a finite word produced by the strategy $\stratA$ then any sequence of det-breakpoints of $u$ has length smaller than $N$.
\end{lemma}

\begin{proof}
Let $N=|M|\cdot |Q_r|+2$, and consider a partial run $\iotar \xrightarrow[]{a_1} p_1 \xrightarrow[]{a_2}  p_2\xrightarrow[]{a_3}\dots \xrightarrow[]{a_{l}} p_l$ of $\Ar$ on a finite word $u=a_1,\dots, a_l$ that is generated by $\stratA$. Assume toward contradiction that $u$ has $N$ det-breakpoints $i_1<i_2<\dots<i_N$, and let $m_j$ be the memory state of $\stratA$ at step $i_j$.

By the choice of $N$, there must be $j<t\in[1,N]$, such that $(m_j,p_j)=(m_t,p_t)$.
This means that when reaching $p_t$, Eve can repeat the play from $p_j$ to $p_t$, forcing $\stratA$ to produce the same letters $a_{i_j+1}\dots a_{i_t}$ in a loop, producing an infinite word $w$. Moreover, each occurrence of this loop contains a det-breakpoint, so $w$ contains infinitely many det-breakpoints.
By Lemma \ref{lem:safedet}, it follows that $w\notin L(\Ar)$. This contradicts the fact that $\stratA$ is winning in the letter game, as $\stratA$ must always produce a word from $L(\Ar)$ in order to win.
\end{proof}


\subsection{Limit Strategy $\sigmainf$}

Recall that by Lemma \ref{lem:ktokens}, Eve wins $G_k(\Ar)$ for all $k\in\mathbb N$. Let $\Wk\subseteq \Qr^{k+1}$ be the winning region of Eve in $G_k(\Ar)$, and $\stratE_k$ a winning strategy for Eve in $G_k(\Ar)$ from the initial position $(\iotar;\iotar,\dots,\iotar)$.

\begin{proposition}\label{prop:Wk}
Let $(p;q_1,q_2,\dots,q_k)\in \Wk$, let $i\in[1,k]$, and let $\pi_i:[1,i]\to[1,k]$ be an injective function.
Then $(p;q_{\pi_i(1)},q_{\pi_i(2)},\dots,q_{\pi_i(i)})\in W_i$.
\end{proposition}
\begin{proof}
Straightforward.
\end{proof}

\begin{lemma}\label{lem:sigmainf}
There is a strategy\footnote{In \cref{ap:Preliminaries}, we formally defined a ``strategy'' with respect to a specific game. Here we abuse the term ``strategy'' to refer to a general total function on finite words.} $\sigmainf: \Sigma^*\to \Qr$, such that for all $u\in\Sigma^*$, if $\delr^*(u)=\{q_1,q_2,\dots,q_{|\Qr|}\}$, then we have $(\sigmainf(u);q_1,\dots,q_{|\Qr|})\in W_{|\Qr|}$.
\end{lemma}

Notice that in the above definition the cardinality of $\delr^*(u)$ might be smaller than $|\Qr|$ and then some states $q_1,\ldots,q_{|\Qr|}$ repeat.

\begin{proof}
We build $\sigmainf$ by induction on $u$, starting with $\sigmainf(\varepsilon)=\iotar$.

Let us define a strategy $\taukunif:\Qr^k\times\Sigma\to \Qr^k$ for moving $k$ tokens in $\Ar$, by dispatching them uniformly at each nondeterministic choice (remaining tokens are dispatched arbitrarily, for instance using some fixed order on the states). For instance if a state $p$ contains $10$ tokens, and its possible transitions on a letter $a$ are $\delta(p,a)=\{q_1,q_2,q_4\}$, then $\taukunif$ can send $4$ tokens to $q_1$, $3$ tokens to $q_2$, and $3$ tokens to $q_4$.
Let us define a strategy $\sigmakunif:\Sigma^*\to \Qr$ for Eve in the letter game on $\Ar$, as follows.
The memory $M=\Qr^k$ of $\sigmakunif$ consists of $k$ tokens, updated according to $\taukunif$.
The choices made by $\sigmakunif$ are then simply the choices made by $\sigma_k$ against these $k$ tokens.
More formally, $\sigmakunifM: \Qr\times M\times \Sigma\to \Qr$ is defined by $\sigmakunifM(p,m,a)=\sigma_k(p,m,a)$, and its update fuction is induced by $\taukunif:M\times \Sigma\to M$.
The strategy $\sigmakunif:\Sigma^*\to \Qr$ is then defined from $\sigmakunifM$ in a canonical way, using initial memory state $m_0=(\iotar,\dots,\iotar)$, and initial state $\sigmakunif(\epsilon)=\iotar$.


We will preserve the following invariant while building $\sigmainf$: for every finite word $u$, there is an infinite set $I_u\subseteq\mathbb N$ such that for all $k\in I_u$, $\sigmainf$ yields the same run as $\sigmakunif$ on $u$.
This invariant guarantees the statement of the lemma (using Proposition \ref{prop:Wk}), since as soon as $k$ is big enough, all states from $\delr^*(u)$ are each reached by $|\Qr|$ tokens when playing $\taukunif$, and $\sigmakunif$ must always stay in the winning region $\Wk$.

We start with $I_\varepsilon=\mathbb N$, for which the invariant trivially holds.

Assume it holds for $u$ with some infinite set $I_u$, and let $a\in\Sigma$. Let $p=\sigmainf(u)$. For each $k\in\mathbb N$, let $p_k=\sigmakunif(u)$. There exists $q\in \Qr$ such that for infinitely many $k\in I_u$, we have $p_k=q$. We set $\sigmainf(ua)=q$, and $I_{ua}=\{k\in I_u\mid p_k=q\}$.

This maintains the invariant, and thus we can conclude the proof by induction.
\end{proof}

\subsection{Playing Against $\tau$}
\label{ssec:playing}

We will now describe a strategy $\stratE$ for Eve in the letter game of $\Ar$, so that the play yielded by $\stratE$ playing against $\stratA$ is winning for Eve. This will contradict the assumption that $\stratA$ is a winning strategy, leading to the conclusion that $\Ar$ is GFG.

Let $N$ be the constant from \cref{lem:taubreak}. 
The strategy $\stratE$ will intuitively play the $N$-tokens game in $\A_r$ against $N$ imaginary \emph{main tokens} $q_1$, $q_2$, \ldots $q_N$. Here ``imaginary'' means that these tokens exist only in the memory of Eve, and are not part of the actual game arena. So if $u$ is the finite word read so far and $p$ is the current state of Eve, when $\stratA$ produces a new letter $\letter$, Eve will choose a successor state $p'$ by setting $p'=\stratE_N(u\letter,p,q_1,\dots,q_N)$, where $\stratE_N$ is a winning strategy of Eve in $G_N(\Ar)$. 

If $\stratA$ eventually produces a word $w$ not in $L(\A)$, Eve wins by the definition of the letter game. We may thus consider the case where $w\in L(\A)$. Then, since $\stratE_N$ is a winning strategy for Eve, by the definition of tokens game, either the path produced by $\stratE$ is accepting, which is what we target, or all of the paths generated by the imaginary tokens are rejecting. We shall thus ensure that at least one of the paths generated by a $q_i$ token is accepting.

The $N$ main tokens will aim at producing an accepting path in turns, starting with $q_1$; if $q_1$ seems to fail, moving to $q_2$; and so on; until giving the last chance to $q_N$. At each point of time the index of the \emph{active token} is denoted by $j$, and $q_j$ plays the $|\Qr|$-tokens game on $\Ar$ against yet other $|\Qr|$ imaginary  \emph{deterministic tokens} $d_1$, $d_2$, \ldots $d_{|\Qr|}$. 
That is, the new state of the active token is $q_j'=\stratE_{|\Qr|}(u\letter,q_j, d_1,\dots,d_{|\Qr|})$. Analogously to the previous step, since $\stratE_{|\Qr|}$ is a winning strategy for Eve in the $|\Qr|$-token game on $\Ar$, the path of $q_i$ is guaranteed to accept if at least one path of the deterministic tokens that it plays against is accepting.

Each of the ``awaiting'' main tokens $q_{j+1}, \ldots q_N$ should remain in the ``safe area'' of Eve in the $|\Qr|$-tokens game, namely in $W_{|\Qr|}$, until its turn arrives. This ``waiting in the safe area'' is done according to the strategy $\sigmainf$. That is, for every $i\in[j+1,N]$, we set the new state of the $i$-th main token to $q_i'=\sigmainf(ua)$. 
The ``discarded'' main tokens $q_1,\ldots,q_{j-1}$ proceed arbitrarily to a new state compatible with $\delr$. That is, for every $i\in[1,j-1]$, we set the new state of the $i$-th main token to $q_i'\in\delr(q_i,a)$.  

What did we get so far? Instead of directly producing an accepting run for Eve in her letter game, moving around the token $p$, we aim at producing an accepting path for one of the main tokens $q_1,\ldots,q_N$, which we again reduce to producing an accepting path for one of the deterministic tokens $d_1$, \ldots $d_{|\Qr|}$. What is it good for? The first reduction allows to try out $N$ paths instead of a single one. The second reduction allows not to only consider a connected paths, but also paths with up to $N$ ``jumps'' between co-reachable states. That is, whenever the active token is replaced, namely when the index $j$ of the active token is increased by one, a new token game starts between $q_j$ and the deterministic tokens  $d_1$, \ldots $d_{|\Qr|}$. At this point, each of the deterministic tokens can be changed to a new state not only by following $\delr$ but also by going to any co-reachable state.

The $|\Qr|$ deterministic tokens proceed according to $\deltadet$; if for some token $d_i$, the transition $\deltadet$ is not defined or makes a rejecting transition, the token $d_i$ is no longer ``alive'', and we maintain a set $E\subseteq \Qr$ of the alive deterministic tokens. 
That is, for every $i\in E$, we move the token $d_i$ to $\deltadet(d_i,\letter)$, if this transition of $\deltadet$ is accepting, or to an arbitrary state in $\delr(d_i,\letter)$ otherwise.

If the set $E$ of alive deterministic tokens becomes empty, it is a \emph{breakpoint}, on which $\stratE$ behaves as follows: the active token $q_j$ finishes its turn, and $q_{j+1}$ gets its turn to be the active token and play against the deterministic tokens, which become alive again and are spread across all reachable states in $\Ssafe$. That is, we choose the new states $d_1',d_2',\dots,d_{|\Qr|}'$ of the deterministic tokens in any canonical way such that $\{d_1',d_2',\dots d_{|\Qr|}'\}=\delr^*(ua) \cap \Ssafe$.

To sum up the description of $\stratE$, it uses the infinite memory structure $\Sigma^*\times \Qr^N\times [1,N] \times \Qr^{|\Qr|}\times 2^{[1,|\Qr|]}$, 
where a memory state $m=(u,q_1,\dots, q_N, j,d_1,\dots, d_{|\Qr|},E)$ consists of
\begin{itemize}
\item The prefix $u$ of the word read so far.
\item $N$ main tokens $q_1,\dots,q_N$.
\item The index $j\in[1,N]$ of the currently active main token.
\item $|\Qr|$ deterministic tokens $d_1,\dots,d_{|\Qr|}$.
\item A set $E\subseteq |\Qr|$ of the indexes of the alive deterministic tokens, namely those that encountered only accepting transitions since the last breakpoint.
\end{itemize}

The initial memory state is $m_0=(\varepsilon,\iotar,\dots,\iotar,1,\iotar,\dots,\iotar,\{1\})$, where all tokens are in $\iotar$, the active main token is the first one, and only one deterministic token (of index $1$) is alive.
This memory structure of $\stratE$ is updated as described above, the behaviour of the tokens is illustrated in Fig. \ref{fig:runs}.

\begin{figure}
\centering
\includegraphics[scale=.5]{runs.pdf}
\caption{An illustration of the behaviour of tokens in the memory structure of the strategy $\stratE$. Awaiting main tokens are represented in black, active tokens in green, and alive deterministic tokens in red. Breakpoints are represented by dashed vertical lines.}
\label{fig:runs}
\end{figure}

We are now ready to prove the main theorem stating the correctness of $\stratE$.
\begin{lemma}\label{lem:sigmatau}
The strategy $\stratE$ wins against $\stratA$ in the letter game of $\A$.
\end{lemma}

\begin{proof}
First of all, notice that by the construction of $\stratE$, if $E$ becomes empty while token $q_i$ is active, then the word $u$ produced by $\stratA$ so far has witnessed $i$ det-breakpoints.
By Lemma \ref{lem:taubreak}, this means that we will never run out of main tokens, and eventually an active token $q_i$ stays active forever.

Let us consider the point of the run where this token $q_i$ becomes active, and let $u$ be the word produced so far. At the breakpoint, deterministic tokens are placed such that $\{d_1,d_2,\dots d_{|\Qr|}\}=
\delr^*(ua) \cap \Ssafe$.
Since $q_i$ followed $\sigmainf$ until now, we have $q_i=\sigmainf(u)$.
By Prop. \ref{prop:Wk} and Lemma \ref{lem:sigmainf}, we have $(q_i,d_1,\dots,d_{|\Qr|})\in W_{|\Qr|}$.
From now on, since no more det-breakpoints occur, some deterministic token $d_h$ will never encounter a rejecting transition, and will safely follow $\deltadet$ forever.
Since $q_i$ now moves according to $\stratE_{|\Qr|}$ against $d_1,\dots,d_{|\Qr|}$, and since $d_h$ follows an accepting run, we obtain that $q_i$ will follow an accepting run.

Finally, since the states assigned to $p$ are chosen according to $\stratE_N$ against $q_1,\dots,q_N$, and since $q_i$ follows an accepting run, we have that $p$ follows an accepting run, and thus the play yielded by $\stratE$ against $\stratA$ is winning for Eve.
\end{proof}

Assuming that Eve wins $G_2(\Ar)$ and $\Ar$ is not GFG leads to a contradiction, we can therefore conclude that $\Ar$ is GFG, and thus $\A$ is GFG by \cref{lem:G2RestrictionPreserve,lem:OperationsPreserve}. We finally have shown \cref{thm:G2cobuchi}.

